Multivariate Analysis of Scheduling Fair Competitions

A \emph{fair competition}, based on the concept of envy-freeness, is a non-eliminating competition where each contestant (team or individual player) may not play against all other contestants, but the total difficulty for each contestant is the same: the sum of the initial rankings of the opponents for each contestant is the same. Similar to other non-eliminating competitions like the Round-robin competition or the Swiss-system competition, the winner of the fair competition is the contestant who wins the most games. The {\sc Fair Non-Eliminating Tournament} ({\sc Fair-NET}) problem can be used to schedule fair competitions whose infrastructure is known. In the {\sc Fair-NET} problem, we are given an infrastructure of a tournament represented by a graph $G$ and the initial rankings of the contestants represented by a multiset of integers $S$. The objective is to decide whether $G$ is \emph{$S$-fair}, i.e., there exists an assignment of the contestants to the vertices of $G$ such that the sum of the rankings of the neighbors of each contestant in $G$ is the same constant $k\in\mathbb{N}$. We initiate a study of the classical and parameterized complexity of {\sc Fair-NET} with respect to several central structural parameters motivated by real world scenarios, thereby presenting a comprehensive picture of it.

==> Preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{soul}
\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
\newcommand{\alg}[1]{\mbox{\sf #1}}
\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
% \usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{subfig}
\usepackage[ruled, linesnumbered]{algorithm2e}
\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{todonotes}
\usepackage{vmargin} %changes the margins

\usepackage{algorithmic}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\date{}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\yes}{\textsf{Yes} }
\newcommand{\no}{\textsf{No} }
\newcommand{\yesinstance}{\yes-instance }
\newcommand{\noinstance}{\no-instance }
\newcommand{\tw}{\mathtt{tw} }
\newcommand{\NP}{\textsf{NP} }
\newcommand{\coNP}{\textsf{coNP} }
\newcommand{\coNPpoly}{\textsf{coNP/poly} }
\newcommand{\FPT}{\textsf{FPT} }
\newcommand{\XP}{\textsf{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard }
\newcommand{\NPC}{\textsf{NP}-complete }
\newcommand{\paraH}{\textsf{para-NP}-hard }
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\domain}{\mbox{\sf dom}}
\newcommand{\image}{\mbox{\sf ima}}
\newcommand{\dete}{\mbox{\sf det}}
\newcommand{\sign}{\mbox{\sf sign}}
\newcommand{\rank}{\mbox{\sf rank}}
\newcommand{\rep}[2] {$\widehat{{\mathcal #1}} \subseteq_{rep}^{#2} {\mathcal #1}$}
\newcommand{\bnoml}[2]{ $\binom{{#1}}{{#2}}$}
\newcommand{\cO}{{\mathcal{O}}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}
								
% Names with special chars

% Paper-specific commands
\newcommand{\child}{\mathrm{children}}
\newcommand{\leaf}{\mathrm{leaves}}
\newcommand{\degr}{\mathrm{deg}}	
\newcommand{\vc}{\mathtt{vc}}
\newcommand{\fvs}{\mathtt{fvs}}
% \newcommand{\sfair}{{\sc $S$-Fair Scheduling}}
\newcommand{\sfair}{{\sc Fair Non-Eliminating Tournament}}
\newcommand{\fair}{{\sc Fair-NET}}
\newcommand{\calM}{\mathcal{M}(G,S)}
\newcommand{\sat}{$3$-XSAT$^3_+$ }
\newcommand{\red}[1]{\textcolor{red}{#1}\xspace} 
\newcommand{\orange}[1]{\textcolor{orange}{#1}\xspace}
\newcommand{\remove}[1]{} 
